Stringent limits on $C\!PT$- and Lorentz-invariance violation from $B_s^0$ meson decays

Tests of fundamental symmetries, such as $C\!PT$ and Lorentz invariance, provide sensitive probes of physics beyond the standard quantum-field-theory framework. Possible violations of these symmetries are investigated through interference effects in decays of $B_s^0$ mesons to $D_s^-\pi^{+}$ states. The analysis uses proton-proton collision data collected with the LHCb detector in 2015-2018 at a centre-of-mass energy of $13~\mathrm{TeV}$, corresponding to an integrated luminosity of $6~\mathrm{fb}^{-1}$. The results are interpreted within the Standard Model Extension framework, yielding sensitivities to the Lorentz-violating parameter $\Delta a_{\mu}$ at the ${\cal O}(10^{-14})\,\mathrm{GeV}$ level. Without assuming Lorentz-invariance violation, the $C\!PT$-violating parameter $z$ in the $B_s^0$ system is measured to be $\mathcal{R}e(z) = 0.018 \pm 0.016 \pm 0.003$ and $\mathcal{I}m(z) = 0.003 \pm 0.004 \pm 0.002$, where the first uncertainties are statistical and the second systematic. These results represent the most precise constraints on $C\!PT$ violation in the $B_s^0$ system.

==> Justification.tex <==
\clearpage

\section*{PRL justification}
Using the full \lhcb Run~2 data set, this Letter reports the most precise measurements of \CPT asymmetries and Lorentz-invariance violation in the \Bs system, using \BsToDsPip decays. The results provide the most stringent constraints on such effects in the \Bs sector and offer a sensitive probe of physics beyond the Standard Model. As the first high-precision study of sidereal-time dependence in this system, it establishes a benchmark for future measurements.

==> LHCb/Authorship_LHCb-PAPER-2026-028-arXiv.tex <==
LHCb collaboration:
R. Aaij,
M. Abdelfatah,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin\'en,
T. Ackernley,
A.A. Adefisoye,
B. Adeva,
M. Adinolfi,
P. Adlarson,
C. Agapopoulou,
C.A. Aidala,
S. Akar,
K. Akiba,
H. Al Saleh,
P. Albicocco,
J. Albrecht,
R. Aleksiejunas,
F. Alessio,
P. Alvarez Cartelle,
S. Amato,
J.L. Amey,
Y. Amhis,
Z. Amos,
L. An,
L. Anderlini,
P. Andreola,
M. Andreotti,
S. Andres Estrada,
A. Anelli,
D. Ao,
C. Arata,
F. Archilli,
Z. Areg,
M. Argenton,
S. Arguedas Cuendis,
L. Arnone,
M. Artuso,
E. Aslanides,
R. Ata\'ide Da Silva,
M. Atzeni,
B. Audurier,
J.A. Authier,
D. Bacher,
I. Bachiller Perea,
S. Bachmann,
M. Bachmayer,
J.J. Back,
M. Bai,
Z.B. Bai,
V. Balagura,
A. Balboni,
W. Baldini,
Z. Baldwin,
L. Balzani,
H. Bao,
J. Baptista de Souza Leite,
C. Barbero Pretel,
M. Barbetti,
I.R. Barbosa,
W. Barker,
R.J. Barlow,
M. Barnyakov,
S. Baron,
S. Barsuk,
W. Barter,
J. Bartz,
S. Bashir,
B. Batsukh,
P.B. Battista,
A. Bavarchee,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
N.A. Behling,
S. Belin,
A. Bellavista,
I. Belyaev,
G. Bencivenni,
E. Ben-Haim,
J.L.M. Berkey,
R. Bernet,
A. Bertolin,
L. Bertsch,
F. Betti,
J. Bex,
O. Bezshyyko,
S. Bhattacharya,
M.S. Bieker,
N.V. Biesuz,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J.E. Blank,
S. Blusk,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A. Bohare,
C. Bolognani,
R.B. Bonacci,
A. Bordelius,
F. Borgato,
S. Borghi,
M. Borsato,
J.T. Borsuk,
E. Bottalico,
S.A. Bouchiba,
M. Bovill,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
J.D. Brandenburg,
A. Brea Rodriguez,
N. Breer,
C. Breitfeld,
J. Brodzicka,
J. Brown,
E. Buchanan,
M. Burgos Marcos,
C. Burr,
E. Butera,
C. Buti,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
Y. Cai,
Y. Cai,
A. Caillet,
R. Calabrese,
L. Calefice,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
J.I. Cambon Bouzas,
P. Campana,
A. Campomagnani,
A.C. Campos,
A.F. Campoverde Quezada,
Y. Cao,
S. Capelli,
M. Caporale,
L. Capriotti,
R. Caravaca-Mora,
A. Carbone,
L. Carcedo Salgado,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carus,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
I. Celestino,
S. Cesare,
A.J. Chadwick,
M. Charles,
Ph. Charpentier,
E. Chatzianagnostou,
R. Cheaib,
M. Chefdeville,
C. Chen,
J. Chen,
S. Chen,
Z. Chen,
A. Chen Hu,
M. Cherif,
S. Chernyshenko,
X. Chiotopoulos,
G. Chizhik,
V. Chobanova,
A. Christakakis,
M. Chrzaszcz,
Y. Chu,
V. Chulikov,
P. Ciambrone,
X. Cid Vidal,
P. Cifra,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
C. Cocha Toapaxi,
V. Coco,
A. Codovini,
C.S. Codovini,
J. Cogan,
E. Cogneras,
L. Cojocariu,
S. Collaviti,
P. Collins,
T. Colombo,
M. Colonna,
A. Comerma-Montells,
L. Congedo,
J. Connaughton,
A. Contu,
N. Cooke,
A. Corallo,
G. Cordova,
C. Coronel,
I. Corredoira ,
A. Correia,
G. Corti,
G.C. Costantino,
C. Cotirlan,
J. Cottee Meldrum,
B. Couturier,
D.C. Craik,
N. Crepet,
M. Cruz Torres,
M. Cubero Campos,
E. Curras Rivera,
R. Currie,
C.L. Da Silva,
X. Dai,
J. Dalseno,
C. D'Ambrosio,
G. Darze,
A. Davidson,
O. De Aguiar Francisco,
C. De Angelis,
F. De Benedetti,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
F. De Gregorio,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
A. De Robertis,
E. De Santis,
M. De Serio,
P. De Simone,
F. De Vellis,
J.A. de Vries,
F. Debernardis,
D. Decamp,
S. Dekkers,
L. Del Buono,
B. Delaney,
B. Demaire-Lepape,
J. Deng,
O. Deschamps,
F. Dettori,
B. Dey,
P. Di Nezza,
S. Ding,
Y. Ding,
L. Dittmann,
J.F. Diverchy,
A.D. Docheva,
A. Doheny,
C. Dong,
F. Dordei,
J. Dorta Moreno,
A.C. dos Reis,
J. Dos Santos Oliveira,
A.D. Dowling,
L. Dreyfus,
W. Duan,
P. Duda,
L. Dufour,
V. Duk,
P. Durante,
M.M. Duras,
J.M. Durham,
O.D. Durmus,
K. Duwe,
A. Dziurda,
S. Easo,
E. Eckstein,
U. Egede,
S. Eisenhardt,
E. Ejopu,
L. Eklund,
M. Elashri,
D. Elizondo Blanco,
J. Ellbracht,
S. Ely,
A. Ene,
T. Evans,
F. Fabiano,
S. Faghih,
L.N. Falcao,
B. Fang,
R. Fantechi,
L. Fantini,
M. Faria,
K. Farmer,
F. Fassin,
D. Fazzini,
L. Felkowski,
C. Feng,
M. Feng,
A. Fernandez Casani,
M. Fernandez Gomez,
B. Fernandez Rodino,
J. Fernandez-John,
A.D. Fernez,
F. Ferrari,
F. Ferreira Rodrigues,
R.A. Fini,
R. Fiorenza,
M. Fiorini,
M. Firlej,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
A. Fomin,
M. Fontana,
M. Fontes Vaz,
L.A. Foreman,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Y. Fu,
Q. F\"uhring,
T. Fulghesu,
G. Galati,
M.D. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
M. Gandelman,
P. Gandini,
B. Ganie,
H. Gao,
R. Gao,
T.Q. Gao,
Y. Gao,
Y. Gao,
Y. Gao,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc\'ia Pardi\~nas,
P. Gardner,
L. Garrido,
C. Gaspar,
A. Gavrikov,
J. George,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
S. Ghizzo,
Z. Ghorbanimoghaddam,
F.I. Giasemis,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent\`u,
L. Girardey,
M.A. Giza,
F.C. Glaser,
V.V. Gligorov,
C. G\"obel,
L. Golinka-Bezshyyko,
E. Golobardes,
A. Golutvin,
S. Gomez Fernandez,
A.G. Gomez Mongui,
W. Gomulka,
F. Goncalves Abrantes,
I. Gon\c{c}ales Vaz,
M. Goncerz,
G. Gong,
S. Gong,
J.A. Gooding,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
L.A. Granado Cardoso,
R. Grande Quartieri,
E. Graug\'es,
E. Graverini,
L. Grazette,
G. Graziani,
A.T. Grecu,
N.A. Grieser,
L. Grillo,
C. Gu,
M. Guarise,
L. Guerry,
A.-K. Guseinov,
Y. Guz,
T. Gys,
K. Habermann,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S. Haken,
G. Hallett,
P.M. Hamilton,
Q. Han,
S. Han,
X. Han,
S. Hansmann-Menzemer,
N. Harnew,
T.J. Harris,
L. Hartman,
M. Hartmann,
S. Hashmi,
J. He,
N. Heatley,
A. Hedes,
F. Hemmer,
C. Henderson,
R. Henderson,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
A. Henrot,
J. Herd,
P. Herrero Gascon,
J. Heuel,
A. Heyn,
A. Hicheur,
G. Hijano Mendizabal,
J. Horswill,
R. Hou,
Y. Hou,
D.C. Houston,
N. Howarth,
W. Hu,
X. Hu,
W. Hulsbergen,
R.J. Hunter,
D. Hutchcroft,
M. Idzik,
P. Ilten,
A. Iohner,
S. Jacevicius,
H. Jage,
S.J. Jaimes Elles,
S. Jakobsen,
T. Jakoubek,
E. Jans,
A. Jawahery,
C. Jayaweera,
A. Jelavic,
V. Jevtic,
Z. Jia,
E. Jiang,
X. Jiang,
Y. Jiang,
Y.J. Jiang,
E. Jimenez Moya,
N. Jindal,
M. John,
A. John Rubesh Rajan,
D. Johnson,
C.R. Jones,
S. Joshi,
B. Jost,
J. Juan Castella,
N. Jurik,
I. Juszczak,
K. Kalecinska,
D. Kaminaris,
S. Kandybei,
M. Kane,
Y. Kang,
C. Kar,
M. Karacson,
A. Kauniskangas,
J.W. Kautz,
M.K. Kazanecki,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
S. Kholodenko,
V. Kholoimov,
G. Khreich,
F. Kiraz,
T. Kirn,
V.S. Kirsebom,
N. Kleijne,
A. Kleimenova,
D. Klekots,
K. Klimaszewski,
M.R. Kmiec,
T. Knospe,
R. Kolb,
S. Koliiev,
L. Kolk,
A. Konoplyannikov,
P. Kooij,
P. Kopciewicz,
P. Koppenburg,
A. Korchin,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
E. Kowalczyk,
O. Kravcov,
M. Kreps,
W. Krupa,
W. Krzemien,
O. Kshyvanskyi,
S. Kubis,
M. Kucharczyk,
A. Kupsc,
A. Kurzina,
V. Kushnir,
B. Kutsenko,
J. Kvapil,
I. Kyryllin,
D. Lacarrere,
P. Laguarta Gonzalez,
A. Lai,
A. Lampis,
D. Lancierini,
C. Landesa Gomez,
G. Lanfranchi,
C. Langenbruch,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
H. Lee,
R. Lef\`evre,
M. Lehuraux,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
E.D. Lesser,
B. Leverington,
A. Li,
C. Li,
C. Li,
H. Li,
J. Li,
K. Li,
L. Li,
L. Li,
P. Li,
P.-R. Li,
Q. Li,
T. Li,
T. Li,
W. Li,
Y. Li,
Y. Li,
Y. Li,
Z. Li,
Z. Lian,
Q. Liang,
X. Liang,
Z. Liang,
S. Libralon,
A. Lightbody,
J. Lin,
S. Lin,
T. Lin,
R. Lindner,
H. Linton,
R. Litvinov,
D. Liu,
F.L. Liu,
G. Liu,
K. Liu,
S. Liu,
W. Liu,
X. Liu,
Y. Liu,
Y. Liu,
Y.L. Liu,
G. Loachamin Ordonez,
I. Lobo,
A. Lobo Salvia,
A. Loi,
T. Long,
F.C.L. Lopes,
J.H. Lopes,
A. Lopez Huertas,
C. Lopez Iribarnegaray,
Q. Lu,
C. Lucarelli,
D. Lucchesi,
M. Lucio Martinez,
Y. Luo,
A. Lupato,
M. Lupberger,
E. Luppi,
K. Lynch,
J. Lyu,
S. Lyu,
X.-R. Lyu,
H. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
B. Mack,
I. Mackay,
L.M. Mackey,
L.R. Madhan Mohan,
M.J. Madurai,
D. Magdalinski,
J.J. Malczewski,
S. Malde,
L. Malentacca,
G. Manca,
C. Mancuso,
R. Manera Escalero,
A. Mangalasseri,
F. Manganella,
R. Mangrulkar,
D. Manuzzi,
S. Mao,
D. Marangotto,
J.F. Marchand,
R. Marchevski,
U. Marconi,
L. Mareso,
E. Mariani,
S. Mariani,
C. Marin Benito,
J. Marks,
A.M. Marshall,
L. Martel,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
C. Martinez,
A. Martinez Armas,
D. Martinez Gomez,
D. Martinez Santos,
F. Martinez Vidal,
A. Martorell i Granollers,
A. Massafferri,
R. Matev,
A. Mathad,
C. Matteuzzi,
K.R. Mattioli,
L. Matzner,
A. Mauri,
E. Maurice,
J. Mauricio,
P. Mayencourt,
J. Mazorra de Cos,
M. Mazurek,
D. Mazzanti Tarancon,
M. McCann,
N.T. McHugh,
A. McNab,
R. McNulty,
B. Meadows,
S.E.R. Medaer,
D. Melnychuk,
D. Mendoza Granada,
P. Menendez Valdes Perez,
F.M. Meng,
M. Merk,
A. Merli,
L. Meyer Garcia,
D. Miao,
H. Miao,
S. Mico,
M. Mikhasenko,
D.A. Milanes,
A. Minotti,
E. Minucci,
B. Mitreska,
D.S. Mitzel,
R. Mocanu,
A. Modak,
L. Moeser,
R.D. Moise,
E.F. Molina Cardenas,
T. Momb\"acher,
M. Monk,
T. Monnard,
S. Monteil,
A. Morcillo Gomez,
G. Morello,
M.J. Morello,
M.P. Morgenthaler,
A. Moro,
J. Moron,
W. Morren,
A.B. Morris,
A.G. Morris,
R. Mountain,
Z. Mu,
N. Muangkod,
E. Muhammad,
F. Muheim,
M. Mulder,
K. M\"uller,
F. Mu\~noz-Rojas,
V. Mytrochenko,
P. Naik,
T. Nakada,
R. Nandakumar,
G. Napoletano,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
J. Nicolini,
D. Nicotra,
E.M. Niel,
L. Nisi,
Q. Niu,
B.K. Njoki,
P. Nogarolli,
P. Nogga,
J. Nombela Royo,
C. Normand,
A. Novo Cal,
J. Novoa Fernandez,
G. Nowak,
H.N. Nur,
A. Oblakowska-Mucha,
T. Oeser,
O. Okhrimenko,
R. Oldeman,
F. Oliva,
E. Olivart Pino,
M. Olocco,
R.H. O'Neil,
J.S. Ordonez Soto,
D. Osthues,
J.M. Otalora Goicochea,
A. Oyanguren,
O. Ozcelik,
F. Paciolla,
A. Padee,
K.O. Padeken,
B. Pagare,
T. Pajero,
A. Palano,
L. Palini,
L. Palombini,
M. Palutan,
C. Pan,
X. Pan,
S. Panebianco,
S. Paniskaki,
L. Paolucci,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
C. Parkes,
D. Parmar,
G. Passaleva,
D. Passaro,
A. Pastore,
M. Patel,
J. Patoc,
C. Patrignani,
A. Paul,
C.J. Pawley,
A. Pellegrino,
J. Peng,
X. Peng,
M. Pepe Altarelli,
S. Perazzini,
H. Pereira Da Costa,
M. Pereira Martinez,
A. Pereiro Castro,
C. Perez,
A. Perez Casas,
P. Perret,
A. Perrevoort,
A. Perro,
M.J. Peters,
A. Petkovic,
K. Petridis,
A. Petrolini,
S. Pezzulo,
J.P. Pfaller,
H. Pham,
L. Pica,
M. Piccini,
L. Piccolo,
B. Pietrzyk,
R.N. Pilato,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V.M. Placinta,
M. Plo Casasus,
T. Poeschl,
F. Polci,
M. Poli Lener,
A. Poluektov,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
K. Popp,
K. Prasanth,
C. Prouve,
D. Provenzano,
V. Pugatch,
A. Puicercus Gomez,
G. Punzi,
J.R. Pybus,
Q. Qian,
W. Qian,
N. Qin,
R. Quagliani,
R.I. Rabadan Trejo,
B. Rachwal,
R. Racz,
J.H. Rademacker,
M. Rama,
M. Ram\'irez Garc\'ia,
V. Ramos De Oliveira,
M. Ramos Pernas,
G. Ramsey,
M.S. Rangel,
G. Raven,
M. Rebollo De Miguel,
F. Redi,
J. Reich,
F. Reiss,
Z. Ren,
P.K. Resmi,
M. Ribalda Galvez,
R. Ribatti,
G. Ricart,
D. Riccardi,
S. Ricciardi,
K. Richardson,
M. Richardson-Slipper,
F. Riehn,
K. Rinnert,
P. Robbe,
G. Robertson,
E. Rodrigues,
A. Rodriguez Alvarez,
E. Rodriguez Fernandez,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
J. Roensch,
A. Rogovskiy,
D.L. Rolf,
P. Roloff,
A. Romano,
V. Romanovskiy,
A. Romero Vidal,
G. Romolini,
F. Ronchetti,
T. Rong,
W. Rose,
M. Rotondo,
M.S. Rudolph,
G. Ruggiero,
M. Ruiz Diaz,
J. Ruiz Vidal,
J. Ruz Armendariz,
J.J. Saavedra-Arias,
J.J. Saborido Silva,
D. Sahoo,
N. Sahoo,
B. Saitta,
M. Salomoni,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
L. Santoro ,
E. Santovetti,
A. Saputi,
A. Sarnatskiy,
G. Sarpis,
M. Sarpis,
C. Satriano,
A. Satta,
M. Saur,
H. Sazak,
F. Sborzacchi,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
N. Schmidt,
S. Schmitt,
H. Schmitz,
O. Schneider,
A. Schopper,
N. Schulte,
H. Schumacher,
M.H. Schune,
G. Schwering,
B. Sciascia,
A. Sciuccati,
G. Scriven,
I. Segal,
S. Sellam,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
B. Sevilla Sanjuan,
Y. Shang,
D.M. Shangase,
R.S. Sharma,
L. Shchutska,
T. Shears,
S. Shelton,
J. Shen,
Z. Shen,
S. Sheng,
B. Shi,
J. Shi,
Q. Shi,
W.S. Shi,
E. Shmanin,
R. Silva Coutinho,
G. Simi,
S. Simone,
M. Singha,
I. Siral,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
E. Smith,
M. Smith,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
K. Solovieva,
N.S. Sommerfeld,
R. Song,
Y. Song,
Y. Song,
Y.S. Song,
F.L. Souza De Almeida,
G. Souza De Castro,
B. Souza De Paula,
K.M. Sowa,
E. Spadaro Norella,
E. Spedicato,
J.G. Speer,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
M. Stefaniak,
O. Steinkamp,
F. Suljik,
J. Sun,
L. Sun,
M. Sun,
D. Sundfeld,
P. Svihra,
V. Svintozelskyi,
J. Swallow,
K. Swientek,
F. Swystun,
A. Szabelski,
T. Szumlak,
Y. Tan,
Y. Tang,
Y.T. Tang,
M.D. Tat,
J.A. Teijeiro Jimenez,
F. Terzuoli,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
A.R. Thomson-Strong,
R. Thornton,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
T.T. Todorov,
L. Tomassetti,
G. Tonani,
X. Tong,
T. Tork,
L. Torlai,
L. Toscano,
D.Y. Tou,
C. Trippl,
G. Tuci,
N. Tuning,
L.H. Uecker,
A. Ukleja,
A. Upadhyay,
B. Urbach,
A. Usachov,
U. Uwer,
V. Vagnoni,
A. Vaitkevicius,
A. Valassi,
V. Valcarce Cadenas,
G. Valenti,
N. Valls Canudas,
J. van Eldik,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
R. Van Laak,
M. van Veghel,
P. Varrella,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V\'azquez Sierra,
S. Vecchi,
J. Velilla Serna,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Verdoglia,
M. Vesterinen,
W. Vetens,
D. Vico Benet,
P. Vidrier Villalba,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
B. Vivacqua,
F.C. Volle,
D. vom Bruch,
K. Vos,
C. Vrahas,
J. Wagner,
J. Walsh,
N. Walter,
E.J. Walton,
G. Wan,
A. Wang,
B. Wang,
C. Wang,
C. Wang,
C. Wang,
G. Wang,
H. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
N.W. Wang,
X. Wang,
X. Wang,
X. Wang,
X.W. Wang,
Y. Wang,
Y. Wang,
Y. Wang,
Y.H. Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
M. Waterlaat,
N.K. Watson,
D. Websdale,
Y. Wei,
Z. Weida,
J. Wendel,
B.D.C. Westhenry,
A.S. White,
C. White,
M. Whitehead,
E. Whiter,
A.R. Wiederhold,
D. Wiedner,
M.A. Wiegertjes,
C. Wild,
G. Wilkinson,
M.K. Wilkinson,
M. Williams,
M.J. Williams,
M.R.J. Williams,
R. Williams,
S. Williams,
Z. Williams,
F.F. Wilson,
M. Winn,
W. Wislicki,
M. Witek,
L. Witola,
T. Wolf,
E. Wood,
G. Wormser,
S.A. Wotton,
H. Wu,
J. Wu,
T. Wu,
X. Wu,
Y. Wu,
Z. Wu,
K. Wyllie,
S. Xian,
Z. Xiang,
Y. Xie,
T.X. Xing,
A. Xu,
L. Xu,
M. Xu,
R. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
S. Yadav,
K. Yang,
X. Yang,
Y. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
H. Yeung,
H. Yin,
X. Yin,
C.Y. Yu,
J. Yu,
K. Yu,
X. Yuan,
Y Yuan,
S. Zalambani,
J.A. Zamora Saa,
F. Zangari,
M. Zavertyaev,
M. Zdybal,
F. Zenesini,
C. Zeng,
M. Zeng,
S.H Zeng,
C. Zhang,
C. Zhang,
D. Zhang,
J. Zhang,
L. Zhang,
Q.Z. Zhang,
R. Zhang,
S. Zhang,
S.L. Zhang,
Y. Zhang,
Z. Zhang,
J. Zhao,
M. Zhao,
Y. Zhao,
A. Zhelezov,
S.Z. Zheng,
X.Z. Zheng,
Y. Zheng,
T. Zhou,
X. Zhou,
V. Zhovkovska,
L.Z. Zhu,
X. Zhu,
X. Zhu,
Y. Zhu,
V. Zhukov,
J. Zhuo Gao,
T. Zies,
D. Zuliani,
X. Zuo

==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) LHCbInternal/$(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) LHCbInternal/$(MAIN)-prl && $(LATEX) LHCbInternal/$(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' LHCbInternal/main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && sh LHCbInternal/wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) LHCbInternal/$(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) LHCbInternal/$(MAIN)-prl && $(LATEX) LHCbInternal/$(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex)  $(wildcard */*.tex) $(wildcard */*.bib) $(wildcard */*.bst)
FIGSOURCES = $(wildcard Figures/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) LHCbInternal/$(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl LHCbInternal/$(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prl.pdf $(MAIN)-prlNotes.bib

# remove output file
rmout: 
	rm -f LHCbInternal/$(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

